Enhancing the Performance of DeepReach on High-Dimensional Systems through Optimizing Activation Functions

With the continuous advancement in autonomous systems, it becomes crucial to provide robust safety guarantees for safety-critical systems. Hamilton-Jacobi Reachability Analysis is a formal verification method that guarantees performance and safety for dynamical systems and is widely applicable to various tasks and challenges. Traditionally, reachability problems are solved by using grid-based methods, whose computational and memory cost scales exponentially with the dimensionality of the system. To overcome this challenge, DeepReach, a deep learning-based approach that approximately solves high-dimensional reachability problems, is proposed and has shown lots of promise. In this paper, we aim to improve the performance of DeepReach on high-dimensional systems by exploring different choices of activation functions. We first run experiments on a 3D system as a proof of concept. Then we demonstrate the effectiveness of our approach on a 9D multi-vehicle collision problem.

==> sections/4_proposed_approach__.tex <==
DeepReach uses a deep neural network with 3 hidden layers, each containing 512 nodes, to approximate the value function. The input layer and the 3 hidden layers utilize a sinusoidal activation function.

The choice of activation function can significantly impact a neural network's performance and training time. While the sinusoidal activation function has demonstrated superior performance, it is also more computationally demanding than the popular Relu activation function. To balance the trade-off between speed and performance, we investigate different combinations of activation functions in each layer to achieve optimal performance while minimizing training time.

We first run experiments on a 3D system as proof of concept. Then, we turn to a 9D multi-vehicle collision system, where traditional BRT solvers struggle to find a solution and analytical computation is not feasible. Therefore, our neural network lacks a formal way to test the accuracy of the results. To address this issue, we implement a method for interpreting and validating the neural network's output.

% Overall, our work explores the use of different activation functions to improve the performance and training time of neural networks, while also developing a novel approach for applying neural networks to complex reachability problems.

\subsection{Intertwined Activation Functions}

The Relu activation function is one of the easiest for a neural network to optimize, and a Sine function is usually harder. Therefore, we combine the efficiency brought by the Relu with the performance produced by the Sine activation function. We first fix our neural network structure to be 1x3x1 (1 input layer, 3 hidden layers, and 1 output layer same as the structure used in DeepReach. We also fix the epoch size to 120000 starting with the air3D problem and then moving on to 150000 epochs for the multi-vehicle collision problem. 

For our experiment, we treat two parameters of the neural network as variables: the number of Sine layers and the arrangement of Sine layers. We use all Sine and all ReLU layers as our baselines.

% \subsection{Concatenated Activation Functions}

% Alternatively, we also try to combine the two activation functions. We used a hybrid activation function that switches between the Relu and Sine activation functions. The hybrid function is defined as follows:

% \begin{equation}
% \begin{split}
% \text{if }x < 0: &\quad f(x) = relu(x) \\
%  \text{else}: &\quad f(x) = sin(x)
% \end{split}
% \end{equation}


% We used this hybrid function as the activation function for the hidden layers of the neural network.

\subsection{Result Evaluation}

Validating the accuracy of the computed set is challenging, especially for high-dimensional systems where finding the ground truth of the reachable set is impossible. In this section, we propose a similar method as the scenario optimization proposed in the work of \cite{b9}.

In this method, we sample a finite number of states uniformly across the spectrum of the entire state space. We then apply optimal control $u^*(x)$ (Equation \ref{eqn:5}) and optimal disturbance $d^*$ on each sample state and generate trajectory $\xi_{x, t}^{u, d}(s)$ until $t=T_f$. We define \textbf{violation rate} as the ratio of the number of violations to the total number of sampled states. In our work, we sample 100K states in each experiment.

There are two conditions that can be treated as a violation: 

1) $$\exists x \in BRT^C \land s \in [0, T_f] : \xi_{x, t}^{u, d}(s) \in T$$

2) $$\exists x \in BRT : \forall s \in [0, T_f],  \xi_{x, t}^{u, d}(s) \notin T$$

The first condition says that any state outside of the BRT should not traverse the failure set at any time on the trajectory. The second condition says that any state sampled inside the BRT should intersect the failure set, or else will be treated as a violation. 

The second metric we use to evaluate the model is $\delta_{\tilde{V}, \tilde{\pi}}$, defined as the maximum learned value of an empirically unsafe initial state under the induced policy $\tilde{\pi}$ :

\begin{equation}
\delta_{\tilde{V}, \tilde{\pi}}:=\max _{x \in X}\left\{\tilde{V}(x, 0): J_{\tilde{\pi}}(x, 0) \leq 0\right\}
\end{equation}

where $J_{\tilde{\pi}}(x, 0)$ is the cost function associated with the trajectory obtained by using the policy $\tilde{\pi}(x, t)$ from an initial state $x$ and initial time $t=0$ until $T_f$. Here on, we use $\delta$ as a shorthand for $\delta_{\tilde{V}, \tilde{\pi}}$ for brevity purposes.

Intuitively, the violation rate measures how often the model deviates from the true BRT, and $\delta$-level measures how far away the worst violating state is from the true BRT.

